Efficient Data Analytics on Augmented Similarity Triplets

Data analysis require a pairwise proximity measure over objects. Recent work has extended this to situations where the distance information between objects is given as comparison results of distances between three objects (triplets). Humans find the comparison tasks much easier than the exact distance computation and such data can be easily obtained in big quantity via crowd-sourcing. In this work, we propose triplets augmentation, an efficient method to extend the triplets data by inferring the hidden implicit information form the existing data. Triplets augmentation improves the quality of kernel-based and kernel-free data analytics. We also propose a novel set of algorithms for common data analysis tasks based on triplets. These methods work directly with triplets and avoid kernel evaluations, thus are scalable to big data. We demonstrate that our methods outperform the current best-known techniques and are robust to noisy data.

==> test.tex <==
%% KERNEL PCA PLOTS %%%
	
	\pgfplotsset{title style={at={(0.82,-0.1)}}}
	\pgfplotsset{compat=1.5}
	\noindent
	\begin{figure}[h!]
		\centering\footnotesize
		\begin{tikzpicture}
		\begin{axis}[title={\textsc{mnist}},
		height=0.35\columnwidth, width=0.55\columnwidth, grid=major,
		ymin=5, ymax=100,
		legend columns=-1,
		legend style={
			column sep=1ex,
		},
		ylabel style={align=center},
		ylabel={Purity \%},
		xtick={1,5,10,20,30},
		]
		\addplot+[blue, mark size=1.5pt, mark=square*, mark options={blue}] table[x={x},y={K_10}, col sep=comma]{Data/mnist500KPCA.csv};
		\addplot+[red, dashed, mark size=1.5pt, mark=square*, mark options={red}] table[x={x},y={K_10_aug}, col sep=comma]{Data/mnist500KPCA.csv};
		\end{axis}
		\end{tikzpicture}
		\begin{tikzpicture}
		\begin{axis}[title={\textsc{iris}},
		height=0.35\columnwidth, width=0.55\columnwidth, grid=major,
		ymin=5, ymax=100,
		legend columns=-1,
		legend style={
			column sep=1ex,
		},
		%	legend entries={$\cT(k=5)$, $\cT(k=10)$, $\cT^*(k=5)$, $\cT^*(k=10)$},
		%	%			mark repeat={20},
		%	legend to name=commonlegend,
		yticklabels={,,},xtick={1,5,10,20,30},
		]
		
		\addplot+[blue, mark size=1.5pt, mark=square*, mark options={blue}] table[x={x},y={K_10}, col sep=comma]{Data/irisKPCA.csv};
		\addplot+[red, dashed, mark size=1.5pt, mark=square*, mark options={red}] table[x={x},y={K_10_aug}, col sep=comma]{Data/irisKPCA.csv};
		\end{axis}
		\end{tikzpicture}
		
		\begin{tikzpicture}
		\begin{axis}[title={\textsc{glass}},
		height=0.35\columnwidth, width=0.55\columnwidth, grid=major,
		ymin=5, ymax=100,
		legend columns=-1,
		legend style={
			column sep=1ex,
		},
		xlabel={{\small $\tau\;\%$}},
		ylabel style={align=center},
		ylabel={Purity \%},
		xtick={1,5,10,20,30},
		]
		\addplot+[blue, mark size=1.5pt, mark=square*, mark options={blue}] table[x={x},y={K_10}, col sep=comma]{Data/glassKPCA.csv};
		\addplot+[red, dashed, mark size=1.5pt, mark=square*, mark options={red}] table[x={x},y={K_10_aug}, col sep=comma]{Data/glassKPCA.csv};
		\end{axis}
		\end{tikzpicture}
		\begin{tikzpicture}
		\begin{axis}[title={\textsc{zoo}},
		height=0.35\columnwidth, width=0.55\columnwidth, grid=major,
		ymin=5, ymax=100,
		legend columns=-1,
		legend style={
			column sep=1ex,
		},
		legend entries={$K$, $K^*$},
		%			mark repeat={20},
		legend to name=commonlegend,
		xlabel={{\small $\tau\;\%$}},
		yticklabels={,,},xtick={1,5,10,20,30},
		]
		
		\addplot+[blue, mark size=1.5pt, mark=square*, mark options={blue}] table[x={x},y={K_10}, col sep=comma]{Data/zooKPCA.csv};
		\addplot+[red, dashed, mark size=1.5pt, mark=square*, mark options={red}] table[x={x},y={K_10_aug}, col sep=comma]{Data/zooKPCA.csv};
		\end{axis}
		\end{tikzpicture}	
		\\\tiny\ref{commonlegend}
		\caption{Results show the purity results after applying kernel PCA on the $K$ and $K^*$. Each object is projected to first two principal components of $K$ and $K^*$ and we apply standard k-means clustering on the projected data. The count of clusters is set equal to the number of classes in the datasets.}
		\label{fig:k_pca}
	\end{figure}
